Dr.Occ: Depth- and Region-Guided 3D Occupancy from Surround-View Cameras for Autonomous Driving

3D semantic occupancy prediction is crucial for autonomous driving perception, offering comprehensive geometric scene understanding and semantic recognition. However, existing methods struggle with geometric misalignment in view transformation due to the lack of pixel-level accurate depth estimation, and severe spatial class imbalance where semantic categories exhibit strong spatial anisotropy. To address these challenges, we propose Dr. Occ, a depth- and region-guided occupancy prediction framework. Specifically, we introduce a depth-guided 2D-to-3D View Transformer (D$^2$-VFormer) that effectively leverages high-quality dense depth cues from MoGe-2 to construct reliable geometric priors, thereby enabling precise geometric alignment of voxel features. Moreover, inspired by the Mixture-of-Experts (MoE) framework, we propose a region-guided Expert Transformer (R/R$^2$-EFormer) that adaptively allocates region-specific experts to focus on different spatial regions, effectively addressing spatial semantic variations. Thus, the two components make complementary contributions: depth guidance ensures geometric alignment, while region experts enhance semantic learning. Experiments on the Occ3D--nuScenes benchmark demonstrate that Dr. Occ improves the strong baseline BEVDet4D by 7.43% mIoU and 3.09% IoU under the full vision-only setting.

==> tables/Robustness.tex <==
\begin{table}[t]
    \centering
    \begin{minipage}[c]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/downsample.pdf}
    \end{minipage}%
    \hfill
    \begin{minipage}[c]{0.48\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{l|c|c}
        \hline
        Model & IoU (\%) & mIoU (\%) \\ \hline
        Baseline & 70.36 & 36.01 \\
        \textbf{Dr.Occ} & \textbf{72.87} & \textbf{43.43} \\
        Dr.Occ+Noise & 72.23 & 42.31 \\ \hline
        \end{tabular}}
    \end{minipage}
    \vspace{-5pt} 
    \caption*{\small \textbf{Robustness.} Left: Mask visualization; Right: Noise injection.}
    \vspace{-20pt} 
    \label{tab:combined_robustness}
\end{table}

==> tables/add_depth.tex <==
\begin{table}[t]
  \small
  \centering
  \begin{tabular}{l | c | c c}
      \toprule
      Method & FP Depth & mIoU($\%$) & IoU($\%$) \\
      \midrule
      BEVDet4D (Baseline) & DepthNet & 36.01 & 70.36 \\
      % \hline
      BEVDet4D & MoGe & 18.69 & 60.00 \\
      RGBD-based & DepthNet & 22.97 & 43.49 \\
      % \hline
      Dr.Occ (Ours) & DepthNet & 43.43 & 72.87 \\
  \bottomrule
  \end{tabular}
  \caption{\textbf{Comparison of alternative depth integration strategies on Occ3D-nuScenes.} All methods are built upon BEVDet4D with R50 backbone and 704$\times$256 input resolution. FP Depth denotes the depth source used in forward projection.}
  \label{tab:supp_depth_strategies}
\end{table}


==> tables/additional_ab.tex <==
\begin{table}[t]
  \small
  \centering
  \begin{tabular}{ccc | c c}
      \toprule
      BP & GR & SE & mIoU($\%$) & IoU($\%$) \\
      \midrule
      & & & 36.01 & 70.36 \\
      \checkmark & & & 39.08 & 70.52 \\
      \checkmark & \checkmark & & 41.16 & 71.07 \\
      \checkmark & \checkmark & \checkmark & 41.45 & 71.29 \\
      \bottomrule
  \end{tabular}
  \caption{\textbf{Ablation study on D$^2$-VFormer components.} BP: Backward Projection Densification; GR: depth-guided Geometric Refinement; SE: depth-guided Semantic Enhancement.}
  \label{tab:supp_d2vformer_ablation}
\end{table}

